Design of Light-Matter Interactions for Quantum Technologies

In this Thesis we design radiation patterns capable of creating effective light-matter interactions suited to applications in quantum computing, quantum simulation and quantum sensing. On the one hand, we have used dynamical decoupling techniques to design quantum operations that are robust against errors in environmental and control fields, achieving high-fidelity quantum logic in trapped ions and energy-efficient nuclear magnetic resonance at the nanoscale with nitrogen-vacancy centers in diamond. On the other hand, we have studied generalised models of light-matter interaction, leading to the discovery of selective multi-photon interactions in the Rabi-Stark model and a proposal for preparing non-classical quantum states using the nonlinear quantum Rabi model. Finally, we have shown how the appropriate tailoring of interactions among ultracold atoms in optical lattices could lead to solve the boson sampling problem faster than the best supercomputers, thus demonstrating quantum supremacy. In this manner, we believe the results presented here significantly expand our knowledge on the control of light-matter interactions, and provide optimal scenarios for current quantum devices to generate the next-generation of quantum applications.

==> others/laburpena.tex <==
\addcontentsline{toc}{section}{Laburpena}
\chapter*{Laburpena}


